Design and Electronics Commissioning of the Physics Prototype of a Si-W Electromagnetic Calorimeter for the International Linear Collider

The CALICE collaboration is studying the design of high performance electromagnetic and hadronic calorimeters for future International Linear Collider detectors. For the electromagnetic calorimeter, the current baseline choice is a high granularity sampling calorimeter with tungsten as absorber and silicon detectors as sensitive material. A ``physics prototype'' has been constructed, consisting of thirty sensitive layers. Each layer has an active area of 18x18 cm2 and a pad size of 1x1 cm2. The absorber thickness totals 24 radiation lengths. It has been exposed in 2006 and 2007 to electron and hadron beams at the DESY and CERN beam test facilities, using a wide range of beam energies and incidence angles. In this paper, the prototype and the data acquisition chain are described and a summary of the data taken in the 2006 beam tests is presented. The methods used to subtract the pedestals and calibrate the detector are detailed. The signal-over-noise ratio has been measured at 7.63 +/- 0.01. Some electronics features have been observed; these lead to coherent noise and crosstalk between pads, and also crosstalk between sensitive and passive areas. The performance achieved in terms of uniformity and stability is presented.

==> sections/introduction.tex <==
\section{Introduction}
\label{intro}

The CALICE (Calorimetry for the Linear Collider Experiments) collaboration~\cite{CALICE} is studying several designs of calorimeters for experiments at the future International Linear Collider (ILC)~\cite{ILC}. In order to have a mature design when the first results from the Large Hadron Collider experiments are expected and decisions on future colliders made, two main development phases have been defined. In the first phase, characterised by the construction of ``physics prototypes'', the feasibility of building a pixelised calorimeter is studied. In the second phase, ``technological prototypes'' will focus on the engineering details needed to insert such a calorimeter in an ILC detector. In both phases, the prototypes will be subject to extensive studies at beam test facilities. The mechanical design and data acquisition (DAQ) chain are common to all calorimeters, thereby easing their integration. The physics prototype for the electromagnetic calorimeter (ECAL) described in this document is a high granularity silicon-tungsten sampling calorimeter.

%As documented in the ILC Reference Design Report~\cite{ILC}, physics studies place stringent requirements on the detector, including the ability to measure jet energies with a precision of at least $0.3 / \sqrt{E/GeV}$. It has been demonstrated~\cite{mark} that the Particle Flow Algorithm (PFA)~\cite{PFA} approach to the reconstruction of jet energies in terms of the individual particle positions can achieve this goal for typical jets at the ILC.

%two main beam test rounds have been defined. The first round consists of the construction and testing of ``physics prototypes'', intended to demonstrate the physics performance. One of the physics prototypes for the electromagnetic calorimeter (ECAL) is made of silicon and tungsten, and is described in this document. The second round consists in the construction and testing of ``technological prototypes'', intended to solve real scale mechanics and electronics issues.
%The beam test setup and the commissioning of the detector achieved during 2006, both at DESY and at CERN beam test facilities~\cite{CERN}, are presented.


